JWST Absorption-Line Analysis of UV-Bright Galaxies at $z=7.2-10.6$: Early Chemical Enrichment Traced by C, O, Mg, Al, Si, and Fe

We investigate UV absorption lines tracing cool gas in eight bright ($-21.9 < M_\mathrm{UV} < -20.5$) galaxies at $z=7.2-10.6$ using deep archival JWST/NIRSpec medium-resolution spectra. The eight galaxies were homogeneously selected based on wavelength coverage and data quality from 362 galaxies at $z>7$ available to date, and all eight were observed as part of the SPURS program. We identify multiple absorption lines of low-ionization species (LIS) in five galaxies, while the remaining three show only one or no significant detections. The average LIS equivalent widths $\mathrm{EW}_{\mathrm{LIS}}$ indicate weaker absorption lines in compact ($r_\mathrm{e}\lesssim100$ pc) galaxies with high $L_{\mathrm{H}\beta}/L_{\mathrm{UV}}$ and $\Sigma_{\mathrm{SFR}}$, suggestive of absorption-line suppression due to intense star formation or nuclear activity. We simultaneously fit multiple LIS lines, accounting for both covering fraction $C_f$ and column density $N$, and find that the five galaxies follow the local $C_f$-$N$ relation. Through the LIS-line fitting, we derive chemical abundance ratios. The five galaxies have abundance ratios similar to those of damped Ly$\alpha$ (DLA) systems at $z\sim5-7$ in the [Si/O]-[C/O] and [Fe/Si]-[Al/Si] planes, suggesting that their absorbing gas is similar to that of DLAs. We find that two galaxies at $z\sim7$ are already highly Fe-enriched, with $\mathrm{[Fe/Si]}\simeq-0.2$, near the solar abundance ratio. While the high Fe enrichment may originate from early Type-Ia supernovae (SNe Ia) or pair-instability supernovae (PISNe), these two galaxies also show $\mathrm{[Al/Si]}\sim0$, with no signature of the strong odd-even effect expected from PISNe, in which odd-$Z$ elements are suppressed relative to even-$Z$ elements, favoring SNe Ia.

==> Table/table_template.tex <==
\begin{table*}
    \caption{Caption.}
    \begin{tabular}{cccccccc}
    \hline
    \hline
    Name & R.A. \\ 
    (1) & (2) & (3) & (4) & (5) & (6) & (7) & (8)\\
    \hline
         &  \\
         & \\
    \hline
    \end{tabular}
    \par
    \vspace{0.02\hsize}
    \footnotesize{(1): Name.}
    \label{tab:template}
\end{table*}
